Quantifying social organization and political polarization in online platforms

Optimism about the Internet's potential to bring the world together has been tempered by concerns about its role in inflaming the 'culture wars'. Via mass selection into like-minded groups, online society may be becoming more fragmented and polarized, particularly with respect to partisan differences. However, our ability to measure the social makeup of online communities, and in turn understand the social organization of online platforms, is limited by the pseudonymous, unstructured, and large-scale nature of digital discussion. We develop a neural embedding methodology to quantify the positioning of online communities along social dimensions by leveraging large-scale patterns of aggregate behaviour. Applying our methodology to 5.1B Reddit comments made in 10K communities over 14 years, we measure how the macroscale community structure is organized with respect to age, gender, and U.S. political partisanship. Examining political content, we find Reddit underwent a significant polarization event around the 2016 U.S. presidential election, and remained highly polarized for years afterward. Contrary to conventional wisdom, however, individual-level polarization is rare; the system-level shift in 2016 was disproportionately driven by the arrival of new and newly political users. Political polarization on Reddit is unrelated to previous activity on the platform, and is instead temporally aligned with external events. We also observe a stark ideological asymmetry, with the sharp increase in 2016 being entirely attributable to changes in right-wing activity. Our methodology is broadly applicable to the study of online interaction, and our findings have implications for the design of online platforms, understanding the social contexts of online behaviour, and quantifying the dynamics and mechanisms of online polarization.

==> important-cut-material.tex <==
Our approach differs from prior work examining cultural structure and polarization in online platforms in three main ways. 
Most importantly, our methodology quantifies the cultural makeup of communities in a purely behavioral fashion. 
Communities are similar to each other if and only if their user bases are surprisingly similar; by computing this similarity along a cultural dimension (e.g.\ U.S.\  political partisanship), we can recover an accurate estimate of whether a particular community’s user base is more behaviourally aligned with the left or right end of the spectrum (e.g. the left or right wing of U.S.\ politics). 
Users ``vote with their feet'' to decide the cultural orientation of communities: only action, across large numbers of people, matters. 
In this way, we avoid biases that result from self-reported data, expert labels, and survey-based methods. 
Self-reported data can be subject to social desirability bias, where users may over-report or under-report community memberships according to their perceived social value~\cite{van2008faking}, as well as response bias, as those who opt to report cultural affiliations may differ systematically from the population as a whole~\cite{arnold1981social}. 
Expert labels of community affiliations are subject to labeler bias, and may be less accurate for communities with implicit cultural associations.  
Additionally, community leaders could be incentivized to manipulate the perception of their community's cultural alignment, and thus the community descriptions they write may not accurately represent the makeup of their membership. 
Leveraging the aggregate behavior of community members rather than relying on labeled data avoids this problem. 
Survey methods can suffer from researcher bias, as they may only test for associations that researchers are aware of or interested in~\cite{chenail2011interviewing}, as well as social desirability bias in how participants choose to respond~\cite{krumpal2013determinants}.
Our method quantifies the positions of all communities along our chosen cultural axes, enabling a complete analysis of cultural structure that could uncover previously unknown associations.  

Relatedly, our work builds upon a line of research examining cultural relationships in word embeddings. High-dimensional representations of text, where similar words are positioned close together in the space, have been applied to the study of cultural stereotypes~\cite{garg2018word,bolukbasi2016man,caliskan2017semantics} and the cultural markers of class~\cite{kozlowski2019geometry}. Although our dataset is composed of billions of comments, we do not use the text to create our embedding. Differences in cultural identity are reflected in the words people use, but this relationship is relatively weak for our focus on measuring the cultural orientation of underlying community populations. Communities using similar language may still be culturally distinct, e.g.\ if they discuss similar topics from different viewpoints, and communities with distinct language may still be culturally similar, e.g.\ if they have similar memberships but discuss different topics, or discuss even the same topic in a different language. This discrepancy between the cultural makeup of online communities and the language they use may be especially large for \emph{implicit} associations. For example, our behavioural method scores the membership of the \subreddit{cycling} community, dedicated to `discussion of everything bicycle related', as left-wing, even though explicitly left-wing vocabulary is not particularly prominent in their discussions. 

Finally, previous analyses have studied platforms such as Facebook, Twitter, and Amazon, on which users are guided by algorithmic curation and personalized recommendations~\cite{shi2017millions,del2016echo,conover2011political}. 
As such, traces of user activity on these platforms reflect not only natural human choices but also the influence of underlying algorithms. 
A recent focus has been on examining the effects of algorithmic curation on shaping online cultural structure, e.g.\ measuring the prevalence of algorithmic ``filter bubbles'' of homogeneous content and groups~\cite{pariser2011filter,flaxman2016filter}, but user choices may play even a larger role in shaping this structure~\cite{bakshy2015exposure}. Thus, although our methodology is generally applicable to many online platforms, we apply it here to Reddit, which has maintained a minimalist approach to personalized algorithmic recommendation throughout its history. For many years, there were no algorithmic recommendations directing users to new communities on Reddit~\cite{redditcode}. Even when introduced, they were mostly unpersonalized and relegated to less visible parts of the site design. By and large, when users discover and join communities, they do so through their own exploration---the content of what they see is not algorithmically adjusted to match their previous behaviour. Since the user experience on Reddit is relatively untouched by algorithmic personalization, the patterns of community memberships we observe are more likely the result of user choices, and thus reflective of the cultural structure induced by natural online behaviour. 

==> siguide.tex <==
\texttt{supplementary\_information.pdf}:

Supplementary Table 1: \textbf{Glossary of referenced communities.} Each subreddit is listed along with its description, which is written by the community moderators of the subreddit. Subreddit descriptions were scraped in 2019 and 2020, and as a result, some descriptions are missing for communities which closed or were banned prior to scrape time.

Supplementary Table 2: \textbf{Gender validation data.} Reddit community and American Community Survey occupation pairs used for the \dimension{gender} validation. Some subreddits are mapped to multiple occupations, in which case the average gender ratio is used.
